Time-Frequency Phase Retrieval for Audio -- The Effect of Transform Parameters

In audio processing applications, phase retrieval (PR) is often performed from the magnitude of short-time Fourier transform (STFT) coefficients. Although PR performance has been observed to depend on the considered STFT parameters and audio data, the extent of this dependence has not been systematically evaluated yet. To address this, we studied the performance of three PR algorithms for various types of audio content and various STFT parameters such as redundancy, time-frequency ratio, and the type of window. The quality of PR was studied in terms of objective difference grade and signal-to-noise ratio of the STFT magnitude, to provide auditory- and signal-based quality assessments. Our results show that PR quality improved with increasing redundancy, with a strong relevance of the time-frequency ratio. The effect of the audio content was smaller but still observable. The effect of the window was only significant for one of the PR algorithms. Interestingly, for a good PR quality, each of the three algorithms required a different set of parameters, demonstrating the relevance of individual parameter sets for a fair comparison across PR algorithms. Based on these results, we developed guidelines for optimizing STFT parameters for a given application.

==> convergence_FGLA_long.tex <==

\subsection{Effect of the redundancy on the convergence of FGLA}
\andi{Slim down. Remove first plot, add the main conclusion from it to the text. Hammer down more the main conclusions: 1) We can find the best parameters after few iterations 2) higher redundancies perform equal or better at any time, redundancy 8 yields the best computation time/performance tradeoff}

\label{subsec:comp_convergence}
In this experiment, we investigated the convergence properties of the FGLA~\cite{Perraudin2013griffin}. For this, we analyzed the evolution of the performance of FGLA obtained for various redundancies $D$ and time-frequency width ratios $\lambda$.

A major drawback of iterative phase retrieval algorithms is the necessity to perform several time-consuming iterations. Here, we first evaluate if by changing the redundancy of the STFT, one might be able to reduce the number of iterations needed to achieve a certain result. To do this, we fix $\lambda$ to the best value obtained in Section \ref{subsec:comp_retrieval_algorithms} and recover the phase on the speech dataset using FGLA. We monitored the performance of the algorithm every 10 iterations until the 100th iteration. First, on Fig. \ref{fig:convergence_FGLA}, we see that for redundancies higher than 8, the performance of FGLA is identical at every intermediate step we monitored. Additionally, we see that even after only 10 iterations, the performance of FGLA at redundancy 4 or 8 is higher than at redundancy 2 after 100 iterations. Further, on Fig. \ref{fig:timed_convergence_FGLA} we experiment by performing a different amount of iterations at every redundancy and evaluating the performance not per iteration, but per time in seconds. As higher redundancies have more values, FGLA takes longer to be applied on them. Therefore, in Fig. \ref{fig:timed_convergence_FGLA}, we see that redundancies higher than 8 perform significantly worse than redundancy 8. We also see that when comparing in time, redundancy 8 still obtains the best results at any point in time. This indicates that using FGLA it is preferable to have a higher redundancy of the STFT than to run the algorithm for a longer time. 

Finally, we fix redundancy at 8 and we evaluate the performance of FGLA for different $\lambda$ after 5, 30, 100, and 300 iterations, see Fig. \ref{fig:convergence_FGLA_lambda}. It can be seen that $\mathbf{ODG}$ suffers from ceiling artifacts, and even though it shows an improvement at every measured point, the difference between 100 and 300 iterations is small for the $\lambda$s which already perform well at 100 iterations. On the other side, even for these values the $\mathbf{SNR_{MS}}$ shows a considerable improvement. In conclusion, FGLA continues to improve after 100 iterations, but the analysis of its performance remains stable.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{plots/convergence_PEAQ_FGLA.png}
    \includegraphics[width=0.8\columnwidth]{plots/convergence_SC_FGLA.png}
    \caption{Convergence of FGLA for a given window at five different redundancies. Measured both in terms of $\mathbf{ODG}$ (above) and $\mathbf{SNR_{MS}}$ (below).}
    \label{fig:convergence_FGLA}
\end{figure}

    \begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{plots/convergence_timed_PEAQ.png}
    \includegraphics[width=0.8\columnwidth]{plots/convergence_timed_SC.png}
    \caption{Convergence of FGLA for a given window at five different redundancies. Measured both in terms of $\mathbf{ODG}$ (above) and $\mathbf{SNR_{MS}}$ (below).}
    \label{fig:timed_convergence_FGLA}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\columnwidth]{plots/convergence_lambda_ODG.png}
    \includegraphics[width=0.49\columnwidth]{plots/convergence_lambda_SC.png}
    \caption{Convergence of FGLA for redundancy eight at varying $\lambda$. Measured both in terms of $\mathbf{ODG}$ (left) and $\mathbf{SNR_{MS}}$ (right).}
    \label{fig:convergence_FGLA_lambda}
\end{figure}


==> stft.tex <==
\section{Properties of the STFT}\label{sec:STFT}

  The rich structure of the STFT is particularly apparent in the continuous setting of square-integrable functions, i.e. functions in $\mathbf{L}^2(\RR)$. Thus, we first discuss the core issues that arise in the generation of STFTs within that setting, recalling established theory along the way, and then move to discuss these issues in the setting of discrete STFTs.
  
  \subsection{The continuous STFT}\label{sec:contSTFT}
  
  The STFT of the function $f\in\mathbf{L}^2(\RR)$ with respect to the window $\varphi\in\mathbf{L}^2(\RR)$ is given by 
  \begin{equation}\label{eq:STFTcont}
    \operatorname{V}_\varphi f(x,\omega) = \int_\RR f(t)\overline{\varphi(t-x)}\me^{-2\pi i\omega t}\, dt
  \end{equation}
  The variable $(x,\omega)\in\RR^2$ indicates that $\operatorname{V}_\varphi f(x,\omega)$ describes the time-frequency content of $f$ at time $x$ and frequency $\omega$. The STFT is complex-valued and can be rewritten in terms of two real-valued functions as $\operatorname{V}_\varphi f(x,\omega) = \exp(\textrm{M}_\varphi(x,\omega)+i\mathrm{\phi}_\varphi(x,\omega))$, whenever $\operatorname{V}_\varphi f(x,\omega)\neq 0$. The logarithmic magnitude (\emph{log-magnitude}) $\textrm{M}_\varphi$ is uniquely defined, but the \emph{phase} $\mathrm{\phi}_\varphi$ is only defined modulo $2\pi$.
  Further, while $\textrm{M}_\varphi$ is a smooth, slowly varying function, $\mathrm{\phi}_\varphi$ may vary rapidly and is significantly harder to model accurately. Nonetheless, both functions are intimately related. If $\varphi(t) = \varphi_\lambda(t) := e^{-\pi t^2/\lambda}$ is a Gaussian window, this relation can be made explicit~\cite{po76,auger2012phase} through the phase-magnitude relations
  \begin{equation}\label{eq:origderiv1lam}
  \begin{split}
      \pd{\mathrm{\phi}_{\varphi_\lambda}}{x}(x,\omega) &=
    \lambda^{-1}\pd{\textrm{M}_{\varphi_\lambda}}{\omega}(x,\omega),\\
    %,\quad
  %  \end{equation}
  %\begin{equation} \label{eq:origderiv2lam}
    \pd{\mathrm{\phi}_{\varphi_\lambda}}{\omega}(x,\omega) & = - \lambda\pd{\textrm{M}_{\varphi_\lambda}
    }{x}(x,\omega) - 2\pi x,
    \end{split}
    \end{equation}
    where $\pd{}{\bullet}$ denotes partial derivatives with respect to $\bullet$. Hence, as long as we avoid zeros of $\operatorname{V}_\varphi f$, the phase $\mathrm{\phi}_{\varphi_\lambda}$ can be recovered from $\textrm{M}_{\varphi_\lambda}$ up to a global constant. Since the STFT is invertible, we can recover $f$ from $\textrm{M}_{\varphi_\lambda}$ up to a global phase factor as well, such that it is sufficient to 
    model only the magnitude $\textrm{M}_{\varphi_\lambda}$. 
    
    Note that the partial phase derivatives are of interest by themselves. In contrast to the phase itself, they provide an intuitive interpretation as local instantaneous frequency and time and are useful in various applications~\cite{dolson1986phase,aufl95}. Further, as suggested by \eqref{eq:origderiv1lam}, the phase derivatives might be a more promising modeling target than the phase itself, at least after unwrapping and demodulation\footnote{Formally, demodulation is simply adding $2\pi x$ to $\pd{\mathrm{\phi}_{\varphi_\lambda}}{\omega}(x,\omega)$.} as detailed in \cite{arfib2011time}.
    
    Note that not every function $F\in\mathbf{L}^2(\RR^2)$ is the STFT of a time-domain signal because the STFT operator $\operatorname{V}_\varphi$ maps $\mathbf{L}^2(\RR)$ to a strict subspace of $\mathbf{L}^2(\RR^2)$. Formally, assuming that the window $\varphi$ has unit norm, the inverse STFT is given by the adjoint operator $\operatorname{V}_\varphi^\ast$ of $\operatorname{V}_\varphi$ and we have $\operatorname{V}_\varphi^\ast(\operatorname{V}_\varphi f) = f$ for all $f$. Now, if $F\in \mathbf{L}^2(\RR^2)$ is not in the range of $\operatorname{V}_\varphi$, then $f = \operatorname{V}_\varphi^\ast F$ is a valid time-domain signal, but $F \neq \operatorname{V}_\varphi f$, i.e., $F$ is an \emph{inconsistent} representation of $f$, and the TF structure of $F$ will be distorted in $\operatorname{V}_\varphi f$. %To reduce such distortion when generating signals in the STFT domain, it is helpful to generate consistent representations $F$. 
    
    In the presence of phase information, consistency of $F$ can be evaluated simply by computing the norm difference $\|F-\operatorname{V}_\varphi(\operatorname{V}_\varphi^\ast F)\|$ which can also serve as part of a training objective. 
    If only magnitudes $\widetilde{\textrm{M}}$
    are available, we can theoretically exploit the phase-magnitude relations \eqref{eq:origderiv1lam}, reconstruct the phase, and then evaluate consistency. 
    Unless otherwise specified, coefficients that are not necessarily consistent are indicated by the symbol $\sim$, e.g., generated magnitudes $\widetilde{\textrm{M}}$. 
    In practice, phase recovery from the magnitude $\widetilde{\textrm{M}}$ introduces errors of its own and the combined process may become too expensive to be attractive as a training objective. Thus, it might be preferable to evaluate consistency of the generated magnitude %$\widetilde{\textrm{M}}$ 
    directly, which, for Gaussian windows, can be derived from \eqref{eq:origderiv1lam}
    \begin{equation}\label{eq:consistency_contlam}
     \left(\lambda\tfrac{\partial^2}{\partial x^2} + \lambda^{-1}\tfrac{\partial^2}{\partial \omega^2}\right)\textrm{M}_{\varphi_\lambda}(x,\omega) = - 2\pi.
  \end{equation} 
   
  Note that, although \cite{po76} already observed that $\widetilde{\textrm{M}}$ is an STFT magnitude if and only if \eqref{eq:consistency_contlam} holds (and $e^{\widetilde{\textrm{M}}}$ is square-integrable), our contribution is, to our knowledge, the first to exploit this relation to evaluate consistency. 
  Furthermore, the phase-magnitude relations \eqref{eq:origderiv1lam} and the consistency equivalence 
  \eqref{eq:consistency_contlam} 
  can be traced back to the relation of Gaussian STFTs to a certain space of analytic 
  functions~\cite{bargman1961,complexanalysis78}.
  
  In the context of neural networks, the ultimate goal of the generation process is to obtain a time-domain signal, but we can only generate a finite number of STFT coefficients. Therefore,  it is essential that inversion from the generated values is possible and synthesis of the time-domain signal is robust to distortions. In mathematical terms, this requires a window function $\varphi$ and time and frequency steps $a,b\in\RR^+$ specifying a snug STFT (or Gabor) \emph{frame}~\cite{ch16}. While a comprehensive discussion of STFT frames is beyond the scope of this article, it is generally advisable to match $a,b$ to the width of $\varphi$ and its Fourier transform $\hat{\varphi}$. In the case where both $\varphi$ and $\hat{\varphi}$ are at least remotely bell-shaped, a straightforward measure of their widths are the standard deviations $\sigma_\varphi = \sigma(\varphi/\|\varphi\|_{\mathbf L^1})$ and $\sigma_{\hat{\varphi}} = \sigma(\hat{\varphi}/\|\hat{\varphi}\|_{\mathbf L^1})$. Hence, we expect good results if $a/b = \sigma_\varphi/\sigma_{\hat{\varphi}}$. For Gaussian windows $\varphi_\lambda$, we have $\sigma_{\varphi_\lambda}/\sigma_{\widehat{\varphi_\lambda}} = \lambda$, such that $\lambda$ is often referred to as \emph{time-frequency ratio}. For such $\varphi_\lambda$, the choice $a/b = \lambda$ is conjectured to be optimal\footnote{In the sense of the frame bound ratio, which is a measure of transform stability~\cite{ch16}.} in general~\cite{best03}, and proven to be so for $(ab)^{-1}\in\NN$~\cite{faulhuber2017optimal}. Furthermore, the relations  \eqref{eq:origderiv1lam} and \eqref{eq:consistency_contlam} only hold exactly for the undecimated STFT and must be approximated. For this approximation to be reliable, $ab$ must be small enough. The theory suggests that $ab\leq 1/4$ is generally required for reliable reconstruction of signals from the magnitude alone ~\cite{balan2006signal}. For larger $ab$, the values of the STFT become increasingly independent and little exploitable (or learnable) structure remains. 
   
   These considerations provide useful guidelines for the choice of STFT parameters. In the following, we translate them into a discrete implementation.
   
   \subsection{The discrete STFT}\label{sec:discSTFT}
   
   The STFT of a finite, real signal $s\in\RR^L$, with the \emph{analysis window} $g\in\RR^L$,
   time step $a\in \NN$ and $M \in\NN$ frequency channels is given by 
   \begin{equation}\label{eq:STFT_final}
   \begin{split}
      \operatorname{S}_g(s)[m,n] & = \sum_{l\in \underline{L}} s[l]g[l-na]e^{-2\pi i ml/M},
   \end{split}
   \end{equation}
   for
   $n\in \underline{N}, m\in\underline{M}$, where we denote, for any $j\in\NN$, $\underline{j} = [0,\ldots,j-1]$ and indices are to be understood modulo $L$. Similar to the continuous case, we can write $\operatorname{S}_g(s)[m,n] = \exp(\textrm{M}_g[m,n] + i\mathrm{\phi}_g[m,n])$, with log-magnitude $\textrm{M}_g$ and phase $\mathrm{\phi}_g$. 
   The vectors $\operatorname{S}_g(s)[\cdot,n]\in\CC^N$ and $\operatorname{S}_g(s)[m,\cdot]\in\CC^{M}$ are called the $n$-th (time) segment 
  and $m$-th (frequency) channel of the STFT, respectively. 
  
  Let $b=L/M$. Then, the ratio $M/a = L/(ab)$ is a measure of the transform redundancy and the STFT is overcomplete (or redundant) if $M/a > 1$. If $s$ and $g$ are real-valued, all time segments are conjugate symmetric and it is sufficient to store the first
  $M_{\RR} = \lfloor M/2\rfloor$ channels only, such that the STFT matrix can be reduced to the size $M_{\RR} \times N$. 
  
  The inverse STFT with respect to the \emph{synthesis window} $\tilde{g}\in\RR^L$ can be written as 
  $\tilde{s}[l] = \sum_{n\in\underline{N}} \sum_{m\in\underline{M}}  \operatorname{S}_g(s)[m,n]\tilde{g}[l-na]e^{2\pi iml/M}$, $l\in\underline{L}$. We say that 
  $\tilde{g}$ is a \emph{dual window} for $g$, if $\tilde{s} = s$ for all $s\in\RR^L$ \cite{st98-1,janssen1997continuous,rawe90}.
  
  Note that the number of channels $M$ can be smaller than the number of nonzero samples $L_g$ of $g$, as long as 
  $a$ and $M$ respect the widths of $g$ and its Fourier transform $\hat{g}$ as discussed in Sec. \ref{sec:contSTFT}. This yields $aM \approx L\frac{\sigma_g}{\sigma_{\hat{g}}}$ as a general guideline
  with $\sigma_g = \sigma(g/\|g\|_{\ell^1})$ and $\sigma_{\hat{g}} = \sigma(\hat{g}/\|\hat{g}\|_{\ell^1})$.
  Furthermore, with the redundancy $M/a \geq 4$, there is sufficient dependency between the values of the STFT, e.g., to facilitate magnitude-only reconstruction. In our experience, this choice represents a lower bound for reliability of discrete approximation of \eqref{eq:origderiv1lam}.

  \begin{attn}
  Implementations of STFT in  SciPy and Tensorflow introduce a phase skew dependent on the (stored) window length $L_g$ (usually $L_g\ll L$) and with severe effects on any phase analysis and processing if not accounted for. This can be addressed with the conversion between \eqref{eq:STFT_final} and other conventions presented in the supplementary material~\ref{sec:supp-conventions} and \cite{arfib2011time,ltfatnote042}.
  \end{attn} 
  
  \subsection{Phase recovery and the phase-magnitude relationship}\label{ssec:phaserec}
 
  \begin{figure}[t]
    \centering
    % \includegraphics[scale=0.35]{sines_phases.png}
    \vspace{-16pt}
    \caption{Overview of spectral changes resulting from different phase reconstruction methods. (1) Original log-magnitude, (2-4) log-magnitude differences between original and signals restored with (2) cumulative sum along channels (initialized with zeros), (3) PGHI from phase derivatives (4) PGHI from magnitude only and phase estimated from Eq. \eqref{eq:phase-magnitude}.}
    \label{fig:phaserecs}
    \vspace{-24pt}
  \end{figure}
  
  Let $\partial_\bullet$ denote some discrete partial differentiation scheme. Discrete approximation of the phase-magnitude relationship \eqref{eq:origderiv1lam} results in 
  \begin{equation}\label{eq:phase-magnitude}
    \begin{split}
    \partial_n \mathrm{\phi}_g[m,n] & \approx \frac{aM}{\lambda} \partial_m \textrm{M}_g[m,n],\\
    \partial_m \mathrm{\phi}_g[m,n] & \approx -\frac{\lambda}{aM} \partial_n \textrm{M}_g[m,n] - 2\pi na/M,
    \end{split}
  \end{equation}
  as derived in \cite{pruuvsa2017noniterative}. For non-Gaussian windows $g$, choosing $\lambda = \sigma_g / \sigma_{\hat{g}}$ has shown surprisingly reliable results, but accuracy of \eqref{eq:phase-magnitude} depends on the proximity of the window $g$ to a Gaussian nonetheless. Optimal results are obtained for Gaussian windows at redundancy $M/a = L$. While STFTs with $M/a = 4$ perform decently and are considered in our network architecture. In Section \ref{ssec:consistencyEval} we show that a further, moderate increase in redundancy has the potential to further elevate synthesis quality.
  As an alternative to estimating the phase derivatives from the magnitude, it may be feasible to generate estimates of the phase derivative directly within a generative model.
  
  It may seem straightforward to restore the phase from its time-direction derivative by summation along frequency channels as proposed in \cite{engel2019gansynth}. Even on real, unmodified STFTs, the resulting phase misalignment introduces cancellation between frequency bands resulting in energy loss, see Fig.~\ref{fig:phaserecs}(2) for a simple example. In practice, such cancellations often leads to clearly perceptible changes of timbre\footnote{See \url{http://tifgan.github.io} for examples.}. Moreover, in areas of small STFT magnitude, the phase is known to be unreliable~\cite{balazs2016pole} and sensitive to distortions~\cite{alaifari2019stability,alaifari2017phase,mallat2015phase}, such that it cannot be reliably modelled and synthesis from generated phase derivatives is likely to introduce more distortion. 
  Phase-gradient heap integration~\cite[PGHI]{pruuvsa2017noniterative} relies on the phase-magnitude relations \eqref{eq:phase-magnitude} and bypasses phase instabilities by avoiding integration through areas of small magnitude, leading to significantly better and more robust phase estimates $\widetilde{\mathrm{\phi}}$, see Fig.~\ref{fig:phaserecs}(4). PGHI  often outperforms more expensive, iterative schemes relying on alternate projection, e.g., Griffin-Lim \cite{griffin1984signal,le2010fast,Perraudin2013}, at the phaseless reconstruction (PLR) task. Generally, PLR relies heavily on consistent STFT magnitude for good results. Note that the integration step in PGHI can also be applied if phase derivative estimates from some other source are available, e.g., when training a network to learn time- and frequency-direction phase derivatives. For an example, see Fig. \ref{fig:phaserecs}(3).
  
\subsection{Consistency of the STFT}\label{ssec:consistency}

  The space of valid STFTs with a given window is a lower dimensional subspace of all complex-valued matrices of size $M_{\RR} \times N$ and a given, generated matrix $\widetilde{\textrm{S}}$ may be very far from the STFT of any time-domain signal, even if it \emph{looks} correct. To prevent artifacts, it is important to ensure that $\widetilde{\textrm{S}}$ is \emph{consistent}. Let $\operatorname{iS}_{\tilde{g}}$ denote the inverse STFT with the dual window $\tilde{g}$, see Sec. \ref{sec:discSTFT}. Consistency of $\widetilde{\textrm{S}}$ can be evaluated by computing the \emph{projection error}
  \begin{equation}\label{eq:projection}
    \operatorname{e}^\textrm{proj} = \|\widetilde{\textrm{S}}- \operatorname{S}_g(\operatorname{iS}_{\tilde{g}}(\widetilde{\textrm{S}}))\|, 
  \end{equation}
  where $\|\cdot\|$ denotes the Euclidean norm. When $\operatorname{e}^\textrm{proj}$ is large, its effects on the synthesized signal are unpredictable and degraded synthesis quality must be expected. Although $\operatorname{e}^\textrm{proj}$ is an accurate consistency measure, it can be computationally expensive. Further, its use for evaluating the consistency of magnitude-only data is limited: When preceded by phase recovery, $\operatorname{e}^\textrm{proj}$ is unable to distinguish the error introduced by the employed PLR method from inconsistency of the provided magnitude data. 
  
  As an alternative, we instead propose an experimental measure that evaluates consistency of the log-magnitude directly. The proposed consistency measure exploits the consistency relation \eqref{eq:consistency_contlam}. An approximation in the spirit of \eqref{eq:phase-magnitude} yields
  \begin{equation}\label{eq:laplacian}
    \frac{\lambda}{a^2}\partial_n^2 \textrm{M}_g[m,n] + \frac{M^2}{\lambda} \partial_m^2 \textrm{M}_g[m,n] \approx -2\pi. 
  \end{equation}
  In practice, and in particular at moderate redundancy, we found \eqref{eq:laplacian} to be prone to approximation errors. Experimentally, however, a measure inspired by the sample Pearson correlation~\cite{lyons1991practical} provided promising results. 
  Let $\tilde{\textrm{M}}$ be the generated magnitude, we have
  \begin{equation}
     \textrm{DM}_n = |\partial_n^2 \tilde{\textrm{M}} +  \tfrac{\pi a^2}{\lambda}|,\ 
     \textrm{DM}_m = |\partial_m^2 \tilde{\textrm{M}}s + \tfrac{\pi \lambda}{M^2}|,
  \end{equation}
   where the terms $\pi a^2/\lambda$ and $\pi \lambda/M^2$ are obtained by distributing the shift $2\pi$ in \eqref{eq:laplacian} equally to both terms on the left hand side. We define the consistency $\varrho(\tilde{\textrm{M}})$ of $\tilde{\textrm{M}}$ as
  \begin{equation}\label{eq:logM-consistency}
    \varrho(\tilde{\textrm{M}}) := \operatorname{r}(\textrm{DM}_n,\textrm{DM}_m),
  \end{equation}
  where $\operatorname{r}(X,Y)$ is the sample Pearson correlation coefficient of the paired sets of samples $(X,Y)$. If the equality is satisfied in \eqref{eq:laplacian}, then  $\varrho(\tilde{\textrm{M}})=1$. Conversely if $\varrho(\tilde{\textrm{M}})\approx 0$, then \eqref{eq:laplacian} is surely violated and the representation is inconsistent.  The performance of $\varrho$ as consistency measure is discussed in Section \ref{ssec:consistencyEval} below.
  
  \section{Performance of the consistency measure}\label{ssec:consistencyEval}
  
  The purpose of the consistency measure $\varrho$ is to determine whether a generated log-magnitude is likely to be close to the log-magnitude STFT of a signal, i.e. it is consistent. As discussed above, consistency is crucial to prevent degraded synthesis quality. Hence, it is important to evaluate the dependence of its properties on changes in the redundancy, the window function and its sensitivity to distortion. 
  
  In a first test, we compute the mean and standard deviation of $\varrho$ on a speech and a music dataset, see Section \ref{sec:TiFGAN} for details, at various redundancies, using Gaussian and Hann windows with time-frequency ratio $\lambda \approx 4$ and STFT parameters satisfying $aM/L = 4$, see Fig. \ref{fig:consistency_per_redundancy}. We note that a Gaussian random matrix takes surprisingly high values for $\varrho$ and, thus, $\varrho$ is not reliable below redundancy $4$. For Gaussian windows, mean consistency increases with redundancy, while the standard deviation decreases, indicating that $\varrho$ becomes increasingly reliable and insensitive to signal content. This analysis suggests that a redundancy of $8$ or $16$ could lead to notable improvements. At redundancy $4$, spectrograms for both types of data score reliably better than the random case, with speech scoring higher than music. The Hann window scores worse than the Gaussian on average in all conditions, with a drop in performance above $M/a = 16$. This indicates that $\varrho$ is only suitable to evaluate consistency of  Hann window log-magnitudes for redundancies in the range $6$ to $16$.
\begin{figure}[t]
      \centering
    %   \includegraphics[scale=0.4]{consistency_per_redundancy.pdf}
      \vspace{-0.5cm}
      \caption{Consistency as function of the redundancy for various time-domain windows. Random matrix from Gaussian distribution.}
      \label{fig:consistency_per_redundancy}
    \vspace{-18pt}
\end{figure}

In a second test, we fix a Gaussian STFT with redundancies $4$ and $8$ and evaluate the behaviour of $\varrho$ under deviations from true STFT magnitudes. To this end, we add various levels of uniform Gaussian noise to the STFT before computing the log--magnitude, see Fig. \ref{fig:consistency_noisy_nofloor}. At redundancy $8$ we observe a monotonous decrease of consistency with increasing noise level. In fact, the consistency converges to the level of random noise at high noise levels. Especially for music, $\varrho$ is sensitive to even small levels of noise. At redundancy $4$, the changes are not quite as pronounced, but the general trend is similar. While this is not a full analysis of the measure $\varrho$, it is reasonable to expect that models that match the value of $\varrho$ closely generate approximately consistent log-magnitudes

    \begin{figure}[th!]
      \centering
    %   \includegraphics[scale=0.4]{consistency_noisy_no_floor.pdf}
      \vspace{-0.8cm}
      \caption{Consistency as a function of SNR obtained by adding complex-valued Gaussian noise to the STFT coefficients.}
      \label{fig:consistency_noisy_nofloor}
      \vspace{-0.4cm}
  \end{figure}
  
Furthermore, the results suggest that $\varrho$ has a low standard deviation across data of the same distribution. In the context of GANs, where no obvious convergence criterion applies, $\varrho$ can thus assist the determination of convergence and divergence by tracking 
  \begin{equation}\label{eq:rel_consistency}
      \gamma = \left|\mathbb{E}_{\bf{M} \sim \mathbb{P}_{M_\text{real}}}\left[ \varrho(\bf{M}) \right] - \mathbb{E}_{\bf{M} \sim \mathbb{P}_{M_\text{fake}}}\left[ \varrho(\bf{M}) \right]\right|.
  \end{equation} 

